Accelerated impurity solver for DMFT and its diagrammatic extensions

We present ComCTQMC, a GPU accelerated quantum impurity solver. It uses the continuous-time quantum Monte Carlo (CTQMC) algorithm wherein the partition function is expanded in terms of the hybridisation function (CT-HYB). ComCTQMC supports both partition and worm-space measurements, and it uses improved estimators and the reduced density matrix to improve observable measurements whenever possible. ComCTQMC efficiently measures all one and two-particle Green's functions, all static observables which commute with the local Hamiltonian, and the occupation of each impurity orbital. ComCTQMC can solve complex-valued impurities with crystal fields that are hybridized to both fermionic and bosonic baths. Most importantly, ComCTQMC utilizes graphical processing units (GPUs), if available, to dramatically accelerate the CTQMC algorithm when the Hilbert space is sufficiently large. We demonstrate acceleration by a factor of over 600 (100) in a simulation of $\delta$-Pu at 600 K with (without) crystal fields. In easier problems, the GPU offers less impressive acceleration or even decelerates the CTQMC. Here we describe the theory, algorithms, and structure used by ComCTQMC in order to achieve this set of features and level of acceleration.

==> Src/Implementation_details.tex <==

In this section, we present the various techniques implemented in \ctqmcname{} in order to reduce the computational burden. We divide those techniques into two sections: CPU optimizations and GPU acceleration. In the former, we discuss the general parallelism scheme, the optimization of the various moves made  to explore the configuration spaces, and the algorithms implemented to alleviate the largest bottleneck in CT-HYB calculations: the evaluation of the local trace. In the latter, we discuss the general interface between the CPUs and GPUS and the algorithms and frameworks used to expedite GPU computations and greatly reduce memory requirements. The improvements discussed in this section are limited to the CTQMC portion of the \ctqmcname{} package, as the post-processing code \verb|EvalSim| requires a comparatively negligible amount of computational resources.

\subsection{CPU Optimizations}

Let us begin with a discussion of the CPU parallelism and those algorithms used to increase the efficiency of the CTQMC.

\begin{figure}
\centering
\includegraphics[scale=1]{fig/Parallelism.eps}
\caption{Parallelism in \ctqmcname. A single Markov chain is created on each MPI image (CPU), with one exception: Each available GPU is paired with a CPU. This GPU accelerated CPU creates a (user specified) number of a Markov chains. While the non-accelerated CPUs handle the local trace computation on their own, the accelerated CPUs hand off the matrix algebra required to the GPU. While waiting for the GPU to handle this algebra, the CPU moves onto the next Markov chain which is not waiting for the GPU to finish its work.  }
\label{fig:parallelism}
\end{figure} 

\subsubsection{CPU parallelism}

One of the reasons to use CTQMC is its nearly ideal scaling. That is, one can simulate many, independent Markov chains and then collect the results from each simulation. Very little or no communication between these simulations is required, at least until their results are collected. Therefore, a CTQMC code can simulate one Markov chain per CPU without incurring a substantial performance loss. \ctqmcname{} uses the message passing interface (MPI) to initialize and distribute these Markov chains, collect the results, and compute the average $\eta_[\mathcal{O}$ after thermalization. A small amount of serial code is required before or after these communication events, e.g., to compute the statistics of the results (across the many Markov chains simulated), conduct I/O, and compute the eigenvectors and eigenvalues of the local Hamiltonian. Figure \ref{fig:parallelism} depicts the parallelism scheme with GPU acceleration, which will be discussed in Sec. \ref{sec:CUDA}.

The structure of this parallelism is simple and effective. As no CPU-to-CPU communication occurs during the computationally demanding measurement or thermalisation phases of the CTQMC, \ctqmcname{} scales extremely well with the number of CPUs. Indeed, if the measurement and thermalisation time are long, \ctqmcname{} scales ideally, as shown in Fig. \ref{fig:scaling}(a):  Provided the user does not require measurement across thousands of CPUs within 10 minutes, the scaling remains above 0.95 of the ideal. We reiterate that this feature of CTQMC is one of the reasons it has risen to prominence, and is not unique to \ctqmcname{}.

\begin{figure}
\centering
\includegraphics[scale=1]{fig/Scaling.eps}
\caption{ (a) The scaling of \ctqmcname{} with the number of nodes for two measurement times, and (b) The scaling of various GPU parallelism schemes with the number of Markov chains simulated by each GPU.  Iterations* is the number of iterations per minute computed by a single node without GPU acceleration and the same number of active CPU's. Tests were run on the supercomputer Summit at the Oak Ridge National Laboratory (ORNL), which features nodes with 42 CPU and 6 GPU (7 CPU / GPU).}
\label{fig:scaling}
\end{figure}


\subsubsection{Trace computations}\label{sec:trace}

The bottleneck of any CT-HYB algorithm is the computation of the local trace, provided that the Hilbert space is reasonably large (as in a \textit{d}- or \textit{f}-shell system) and the temperature is not extremely low. A number of algorithms have been developed to reduce the computational resources demanded by these calculations.\cite{haule2007quantum, gull2008continuous, yee2012towards, semon2014lazy, seth2016triqs, shinaoka2014hybridization}. \ctqmcname{} employs the lazy skip-list\cite{semon2014lazy} algorithm to optimize the trace computation.

Here we provide a brief overview of the the lazy skip list optimization; for a detailed description  of these algorithms, we refer the reader to Ref. \cite{semon2014lazy}. First, let us note that the Hilbert space of the local Hamiltonian may be divided into sectors according to the abelian symmetries of the Hamiltonian, i.e., its quantum numbers, and the local operators bring the system from one sector no another, $s_i\rightarrow s_{i+1}$. Second, the local trace may be decomposed into the time-evolution operators, $P_{\tau,s}=e^{-\tau H_{loc,s}}$, and operator matrices, $F_{i,s}$, with elements $(F_{i,s})_{mn}=\langle m_s |d_i|n_s\rangle$ in each sector, where $m_s$ and $n_s$ are states in sector $s$ of the Hilbert space. Within this decomposition, the local trace is reformulated as a sum of traces over a product of matrices. That is,
\begin{align}
w_{loc}(\mathcal{C})=\sum_s \mathrm{Tr} P_{\beta-\tau_k,s_{2k}}F_{i_k,s_{2k}}P_{\tau_k-\tau_k',s_{2k-1}}F^\dagger_{i_k',s_{2k-1}}\cdots F_{i_1,s_1}P_{\tau_1-\tau_1',s_1}F_{i_1',s_0}^\dagger P_{\tau_1',s_0}.
\end{align}
 
In general, only a few operators are inserted into the local trace, which might have hundreds of operators. This means that the majority of the subproducts are left untouched. One can store these subproducts in a data structure to drastically reduce the number of matrix multiplications required, e.g., a balanced binary tree\cite{Gull2011} or a skip-list\cite{semon2014lazy}. Both of these options offer essentially the same performance, $O(log(k))$, but the skip-list is much easier to implement.

Furthermore, one can evaluate the bounds of the local trace rather than the trace itself in order to decide whether a proposed configuration will be accepted. If the proposed  move is accepted, then the local trace must be computed. Otherwise, one can propose a new move. In real materials at low-temperatures, the acceptance rate can be extremely low. Therefore, if it is much faster to evaluate the bounds of the local trace, one can drastically speed up the CTQMC. The bounds are established by taking the some submultiplicative matrix norm of the matrices in the trace and multiplying by a constant. In the lazy-trace algorithm, the norm chosen is the spectral norm in order to capture the drastic variation in the time-evolution operators. 

The lazy-skip list algorithm combines both ideas, and it was shown that it leads to a 30 to 600 time speedup\cite{semon2014lazy}. 

\subsubsection{CTQMC Move optimizations}\label{sec:CTQMCMoveOptimizations}

While the trace calculation is an unavoidable bottleneck in CT-HYB calculations, a substantial amount of computation can be avoided by only proposing moves which have a chance to be accepted. That is, we often know \textit{a priori} whether a move will be rejected, without having to do an expensive local trace computation in addition to the moderately burdensome hybridization and dynamical interaction computations. 

Consider the pair insertion move. In the literature, this move is typically made by generating two random times for the creation and annihilation operator, computing the Metropolis-Hastings acceptance rate, and then deciding to accept or reject the proposed move\cite{Gull2011}, as shown in Fig. \ref{fig:CSCmoves}(a). Often, however, the proposed move will violate the Pauli-exclusion principle, and we have wasted effort computing the acceptance rate. In \ctqmcname, we only propose moves that satisfy the Pauli exclusion principle. In order to accomplish this, we must take extra care with the pair insertion, removal, and worm operator shift moves. Let us briefly outline how we propose the Pauli-aware moves.

\begin{figure}
\centering
\includegraphics[scale=1]{fig/InsertRemove.eps}
\caption{ The (a) standard and (b) Pauli-aware pair insertion and removal moves, where $r_i$ are the random numbers required for the move and $n$ is the number of operators in the current configuration. In the standard algorithm, many randomly proposed moves will be rejected because they generate unphysical configurations. In the Pauli-aware algorithm, the acceptance rate is much higher, particularly at high expansion orders.  }
\label{fig:CSCmoves}
\end{figure}


\textbf{Pair insertion}: First, one selects the flavor of the creation and annihilation operator, $i$ and $j$. Then, we select a random operator from the list of operators of flavor $i$ and $j$ in the current configuration. Next, we generate two random times which lie on the imaginary time axis between this operator and the next operator in the time-ordered list. (If there are no operators in the current configuration of flavor $i$ and $j$, then one simply chooses two random times as in the typical, Pauli-unaware algorithm.) As in the Pauli-unaware algorithm, one must attach a weight to the Metropolis-Hastings acceptance rate in order to maintain the detailed balance. We call that weight the configuration weight, $w_{\mathrm{config}}$. For this Pauli-aware pair insertion move, the configuration weight is
\begin{align}
w_{\mathrm{config}}=\Delta \tau \frac{N}{(N+2)},
\end{align} 
where $\Delta\tau$ is the distance between the pre-existing operators which bound the randomly select times for the newly proposed pair, and $N$ is the number of operators of flavor $i$ and $j$. Note the imaginary time axis is a circle of circumference $\beta$, so that one must take care with the distance calculation and concept of the ``next'' operator. This move is illustrated in Fig. \ref{fig:CSCmoves}(b).

\textbf{Pair removal}: This move proceeds much like the pair insertion move. That is, we select the flavors of the creation and annihilation operators and then select a random operator from the list of operators with these flavors. Then, we select the next operator in the time-ordered list. Finally, we compute the distance between between these pairs along the imaginary time axis, a circle. The resulting configuration weight is
\begin{align}
w_{\mathrm{config}} = \frac{1}{\Delta\tau}\frac{N}{N-2}.
\end{align}
This move is illustrated in Fig. \ref{fig:CSCmoves}(b).

\begin{figure}
\centering
\includegraphics[scale=1]{fig/SwapSplitJoin.eps}
\caption{ The algorithm for moving a local bilinear. In order to generate physical configurations, the bilinear is moved throughout the configuration by swapping one of its operators with a hybridized (configuration space) operator forming a new bilinear at this location, and splitting apart the old bilinear. The operators used for the split and join portions of this move are aware of the Pauli exclusion principle, greatly improving the acceptance rate at large expansion orders.
   }
\label{fig:SwapSplitJoin}
\end{figure}


\textbf{Bilinear swap}: In general, one must swap the location of worm and partition operators in order for the exploration of worm configuration spaces to be ergodic. This is a relatively simple process when one does not  need to swap a bilinear operator: Pauli exclusion is never violated and one only needs to compute the change in the hybridisation.\cite{Gunacker2015} When one swaps one of the operators in a bilinear, however, the other operator in that bilinear must be dealt with carefully. If one simply shifts it, Pauli exclusion will be violated quite often, which might cause ergodicity problems. Moreover, if both operators in a bilinear are swapped, a newly hybridized bilinear is left in place. This hybridized bilinear is relatively unphysical and will therefore typically be rejected by the Metropolis-Hastings algorithm. Again, ergodicity issues arise. Therefore, we must carefully design a smart bilinear swap move. In \ctqmcname, we implement the bilinear swap using a combination swap, join, and split moves in order to avoid the problems outlined above. This move is illustrated in Fig. \ref{fig:SwapSplitJoin}.

As in the typical swap move, the join-swap-split move for a bilinear $n^{(l)}_{ij}$ begins by selecting a random hybridized operator of flavor $i$ ($j$) from the current configuration. This time, $\tau_{\mathrm{join}}$ is where the new bilinear will be placed, and these are the operators which will be swapped (hybridized $\leftrightarrow$ local). 
Then, one finds the operators of flavor $j$ ($i$) which bracket the current and new bilinears. A random time is selected within the operators bracketing the current bilinear, $\tau_{\mathrm{split}}$, and we select the operator of the same type (creation or annihilation) from the operators bracketing the new bilinear. The hybridized operator is moved to $\tau_{\mathrm{split}}$ and the local operator is moved to $\tau_{join}$
The configuration weight associated with this move is 
\begin{align}
w_{\mathrm{config}} = \frac{\Delta \tau_{\mathrm{split}}}{\Delta\tau_{\mathrm{join}}},
\end{align}
where $\Delta\tau_{\mathrm{split}}$ and $\Delta\tau_{\mathrm{join}}$ are the distances between the operators bracketing the original and new bilinears, respectively.

 \subsection{Symmetries of the two-particle correlators}
 
 In general, accurate measurement of the two-particle correlators is much more time consuming than the accurate measurement of the one-particle correlators. In \ctqmcname, we implement a number of symmetries during post-processing which help to improve the accuracy of the measurements. The symmetries implemented in \ctqmcname{} are the Hermetian and Fermionic symmetries, when possible. We list these symmetries in Table \ref{tab:symmetries}
\begin{table}
\caption{Symmetries implemented in \ctqmcname}\label{tab:symmetries}
\begin{center}
\begin{tabular}{c c c}
 \multicolumn{3}{c}{\textbf{Observable}} \\
 $G^{(ph)}_{ijkl}(i\omega)$ & $G^{(pp)}_{ijkl}(i\omega)$ & $G^{(ph)}_{ijkl}(i\nu,i\omega)$  \vspace{1mm} \\
\hline\vspace{2mm}
{$\!\begin{aligned}
&G^{(ph)}_{jilk}(i\omega) \\
&G^{(ph)}_{lkji}(-i\omega) \\
&G^{(ph)}_{klij}(-i\omega)
 \end{aligned}$}
& 
{$\!\begin{aligned}
&G^{(pp)}_{jikl}(i\omega) \\
&G^{(pp)}_{ijlk}(i\omega) \\
&G^{(pp)}_{jilk}(i\omega)
 \end{aligned}$}
&
{$\!\begin{aligned}
&G^{(ph)}_{jilk}(i\omega-i\nu,i\omega) 
 \end{aligned}$} \\
 &&\\
 \multicolumn{3}{c}{\textbf{Observable}} \\
 $G^{(pp)}_{ijkl}(i\nu,i\omega)$  &  \multicolumn{2}{c}{$G^{(ph)}_{ijkl}(i\nu,i\nu',i\omega)$} \vspace{1mm} \\
\hline\vspace{2mm}
{$\!\begin{aligned}
&G^{(pp)}_{ijlk}(i\nu,i\omega) \\
&G^{(pp)}_{jikl}(i\omega-i\nu,i\omega) \\
&G^{(pp)}_{jilk}(i\omega-i\nu,i\omega)
 \end{aligned}$}
 &
 \multicolumn{2}{c}{
{$\!\begin{aligned}
 &G^{(ph)}_{kjil}(i\nu'-i\omega,i\nu',i\nu'-i\nu) \\
 &G^{(ph)}_{ilkj}(i\nu-i\omega,i\nu,i\nu-i\nu') \\
 &G^{(ph)}_{lkij}(i\nu'-i\omega,i\nu-i\omega,i\omega) 
 \end{aligned}$}
 }
 \end{tabular}
 \end{center}
\end{table} 
 
If a symmetric component specified above is not measured (i.e., it is outside the frequency box defined by the user supplied cutoff frequencies), that symmetry is not applied at that frequency. That is, these symmetries are applied whenever possible and ignored otherwise. These symmetries are also implemented for the improved estimators.
 
 \subsection{Asymptotics of the two-particle vertex functions}\label{sec:Asymptotics}
 
If the two-, three-, and four-point, two-particle correlators are measured,  \ctqmcname{} can compute the asymptotic vertex kernel functions. These kernel functions can be used to compute the high frequency domain of the full vertex functions, as described in Ref. \cite{Kaufmann2017}. Without these asymptotics, evaluating the full vertex at even moderate bosonic frequencies is essentially impossible.
 

\subsection{GPU acceleration}\label{sec:CUDA}

\textcolor{blue}{[Slight changes]}
Within CT-HYB algorithms, the inner loop involves taking the product of a large number of matrices. With the lazy-trace algorithm, one must also compute a large number of Frobenious norms. The size of these matrices scales exponentially with the number of orbitals, and the number of matrices which must be multiplied scales with $\beta=1/T$, making the impurity solver prohibitively expensive at low temperatures, particularly $f$-shell systems. In \ctqmcname{}, we use GPUs to handle local trace, i.e., apply the time-evolution operators, multiply the matrices, evaluate the trace, and take the Frobenius norms. Depending on the problem, however, the matrices involved can be small in comparison to the capabilities of a modern GPU, even in an $f$-shell impurity. By developing a bespoke GPU acceleration scheme, we are able to saturate a GPU even in the simplest $f$-shell problems and achieve substantial acceleration. For example, the solution of a simple $f$-shell problem is accelerated by 50x on a single CPU at Summit (or 15x across an entire node). For a more complex $f$-shell problem, i.e., with fewer quantum numbers and imaginary parts in the interaction matrix, we achieve acceleration of a single CPU by over 300x on Summit (or over 40x across an entire node). For the most demanding $f$-shell problems tested, i.e., with only $J^2$ and $N$ as quantum numbers, a GPU accelerates a single CPU by over 500x (or over 70x across an entire node). These more difficult problems were generated using Portobello\cite{Portobello}, which allows one to produce impurities with off-diagonal hybridisation and (complex valued) local Hamiltonian matrices, and complex valued interaction matrices. Without the GPUs, these problems are prohibitively expensive unless an exorbitant number of node hours are thrown at them, particularly in a LDA+DMFT simulation where the impurity problem must be solved O(10) times, or when measuring the susceptibilities, which might require O(1000) times more computation. With GPUs, these problems suddenly become relatively cheap or at least feasible. However, the GPUs do not help with relatively easy problems. Even with our GPU scheme, the matrices in $d$-shell or smaller problems are simply too small. The GPU-CPU communication becomes much more expensive than the matrix multiplications or norm computations within a CPU, and the use of a GPU drastically decelerates the solution. (In these problems, one should set \verb|sim per device| to 0 to avoid using the GPUs: See App. \ref{sec:Installation and Usage}.)

Briefly, let us describe the GPU computation kernels, the most critical of which are the matrix multiplication and Frobenius norm kernels. The matrix multiplication is handled by the CUTLASS library, which works to map the larger problem onto a large number of warp-level matrix multiplication blocks, each grouped into a heirarchy of larger blocks according to the architecture of the device. In general, the performance of the CUTLASS library is very similar to (but very slightly worse than) the cuBLAS libraries. However, it is much more flexible. (The time-evolution operators associated with the matrix multiplications are applied by a blocks of threads with dimension matching the matrix being evolved.) The norm is computed within a block of warps, featuring an optimized reduction within both the block and also the warp. 

Now let us discuss how we mix the CPU and GPU parallelism. Without GPUs, each MPI worker in \ctqmcname{}  controls a single simulation (or Markov chain). With GPUs, there are a number of possible schemes by which to accelerate the time-to-solution. Let us say that we will distribute the available GPUs to each CPU, so that a few CPUs share one GPU. By default, CUDA serializes the usage of the GPU, so that each Markov chain has to wait for the GPU to finish computing a kernels before it continues. With the Multi-Process Service (MPS), CUDA allows the instructions to be carried out in parallel, and the CPUs no longer have to wait for the GPU to finish working on a different Markov chain. However, MPS does not allow the various CPUs to share the global memory of the GPU. So, the GPU must store a copy of the operator matrices for each CPU it accelerates. This limits the GPU: In even the simplest $f$-shell problem, the GPU must store over 0.5 GB of matrices per accelerated CPU. In a more complex problem, the GPU needs to store over 10 GB per CPU. Even on modern GPUs, this drastically limits the number of Markov chains (or CPUs) a GPU can accelerate.
Furthermore, even if the GPU is not limited by the amount of memory required, the matrices involved in CTQMC are often relatively small in comparison to the computational capability of a GPU. Therefore, the GPU will not be saturated when it accelerates a small number of Markov chains.

 CUDA streams offer a paradigm wherein many Markov chains can share the same global memory of the GPU. In combination, MPS and streams allow one to more easily saturate a GPU. For example, we might simulate $n$ Markov chains per $N_{cpu}$ CPUs, such that the GPU handles the computations for $nN_{cpu}$. In this way, we can more easily saturate the GPU. However, we will quickly run out of GPU memory, particularly for more difficult problems or when $N_{cpu}$ is large.

 In \ctqmcname{}, we implement an alternate scheme wherein each GPU is paired with a CPU, and these CPUs control $n$ Markov chains. Each of these Markov chains is placed in a CUDA stream so that the GPU can concurrently handle the impurity trace computations.
   (The remaining, unpaired CPUs handle the trace computations without the help of a GPU, as shown in Fig. \ref{fig:parallelism}.)  Because the GPU can share memory across the CUDA streams, the memory issues associated with MPS are alleviated, and one can simulate a large number of Markov chains per GPU in order to saturate the GPU.  Interestingly, this scheme not only alleviates the memory issues and allows for better GPU saturation, but it also scales better than MPS, as shown in Fig. \ref{fig:scaling}(b). This is particularly true if there are a large number of CPUs per GPU, as in Summit. The scaling is identical to MPS with streams, but we are now free to choose any integer number of Markov chains per GPU (instead of any multiple of the number of CPUs per GPU), and we do not run into memory issues for the more difficult problems. That is, the portability and flexibility of our implementation is much better than MPS with streams, and the performance is strictly better. The major downside to this scheme is the complexity of the programming. Still, it is essential to the success of the GPU acceleration of a flexible CTQMC solver on modern supercomputers.


==> Src/InstallationAndUsage.tex <==
In this section, we describe how one can acquire, install, and use \ctqmcname. \ctqmcname{} is written in C++11 and CUDA, and uses BLAS and LAPACK libraries. It has been tested with GNU, intel, and clang compilers. 

\subsection{Download}

\ctqmcname{} is an open source code distributed under the GNU General Public Licence 3.0 (GPL). It is a part of the COMSUITE package\\ (\verb|https://www.bnl.gov/comscope/software/comsuite.php|), and can therefore be downloaded from the COMSUITE github page\\ (\verb|https://github.com/comscope/comsuite/tree/master/ComCTQMC|). Alternately, one can contact the authors for the current version of \ctqmcname. 

\subsection{Install}

To build \ctqmcname, one must first decompress the downloaded \ctqmcname{} archive. Typically, \ctqmcname{} will be bundled in an archive like \verb|ComCTQMC.tar.gz|. Therefor, one should navigate to the location where this archive resides and execute
\begin{verbatim}
$ tar xvfz ComCTQMC.tar.gz
\end{verbatim}
where \verb|$| is the command line prompt. Then, one must navigate into the extracted directory.
\begin{verbatim}
$ cd ComCTQMC
\end{verbatim}
In this base directory is the file  \verb|Arch.mk| which specifies the compiler options. While default options are setup here, one should manually specify which compiler and libraries one will use. (See the file \verb|Arch.mk| for further information.) 

Once \verb|Arch.mk| has been setup, one must build the CTQMC and post-processing codes. To do so, navigate to the \verb|CTQMC| directory for either the GPU accelerated version (if the system has CUDA enabled GPUs) or the non-accelerated version
\begin{verbatim}
(GPU Accelerated)	$ cd CTQMC/GPU
(Otherwise)				$ cd CTQMC/CPU
\end{verbatim}
and then build the code
\begin{verbatim}
$ make
\end{verbatim}
The post-processing  code \verb|EvalSim| is similarly built:
\begin{verbatim}
$ cd ../../EvalSim
$ make
\end{verbatim}

\subsection{Execute}

To run \ctqmcname, one must first run CTQMC code \verb|CTQMC| and then run the post-processing code \verb|EvalSim|. To do so from the base directory, one would type 
\begin{verbatim}
(GPU Accelerated)	$ CTQMC/GPU/CTQMC params
								$ EvalSim/EVALSIM params
								
(Otherwise)				$ CTQMC/GPU/CTQMC params
								$ EvalSim/EVALSIM params
\end{verbatim}
where the control file is named \verb|params.json|. 

\subsection{Input and output fiiles}
\label{sec:params}


The input and output files are written in the JSON (JavaScript Object Notation) format\footnote{\url{https://www.json.org/}}. Briefly, this format presents a dictionary pairing keys with data.  An entry can store integer, real number, string, boolean,  array (of those types), or another dictionary entry. The order of the dictionary entries does not matter. We will refer to a the highest level entry in the JSON dictionary as a block. Let us describe the input files required by and then output files produced by \ctqmcname{}. 

The following input files are required by \ctqmcname{}:
\begin{enumerate}
\item \verb|params.json|: The control file describing the simulation, the quantum impurity, the desired measurements and worms, and the system architecture.
\item \verb|hybridisation.json|: The hybridisation functions.
\item \verb|dynamical.json| (optional): The dynamical part of the two-body interaction. This is not required if there is no dynamical part. 
\item \verb|config_n.json| (restart): The state of the Markov chain \verb|n| from which to resume a simulation. This can be used to continue a simulation or to reduce thermalisation times.  (Produced by \ctqmcname.)
\item \verb|params.meas.json| (restart): The state of the estimators at the end of the previous run. Required to automatically continue the simulation and refine the estimators.   (Produced by \ctqmcname.) 
\end{enumerate}

After completion, \ctqmcname{} produces the following output files:
\begin{enumerate}
\item \verb|config_n.json|:  The state of the Markov chain $n$ at the end of the run.
\item  \verb|params.meas.json|: The raw measurements needed to compute the observables.
\end{enumerate}

The post-processing code takes these files and produces the following file:
\begin{itemize}
\item  \verb|params.obs.json|: The observables, e.g., the self-energy, four point vertex functions, susceptibilities, and green's functions. 
\end{itemize}

\subsubsection{Input Parameters}

Here we describe the many input parameters in the \verb|params.json| file. As noted previously, these parameters are organized in blocks within the parameter file. We will mirror that organization here, first describing the higher level purpose of that block and then subsequently listing and describing the individual fields within the block. The data type will be given in parenthesis after the name of the field, which is in bold. The default value will be given   after the data type. If there  is no default value, we will write none. If there is no default value, the entry is required. If there is a default value, the entry is optional. The data type matrix is used here to denote an array of arrays.

The miscellaneous parameters which do not belong to their own block are described in Table \ref{tab:params:misc}. The block describing the local Hamiltonian is described in Table \ref{tab:params:hloc}. The block describing the local basis set is described in Table \ref{tab:params:basis}. The block describing the hybridisation between the impurity orbitals and bath is described in Table \ref{tab:params:hybridisation}. The block describing the measurements which occur in partition space are given in Table \ref{tab:params:partition}, while the blocks describing the measurements taken in worm spaces are given in Tables \ref{tab:params:green} and \ref{tab:params:vertex}. Finally, Table \ref{tab:params:kernels} provides the parameters which describe the asymptotic vertex kernels. (This last block is only used during post-processing). 

\ctqmcname{} will only sample a given worm space if the corresponding parameter block is found in the parameter file. Let us briefly discuss the naming scheme used for the worm observable parameter blocks: \textit{green} refers to the one-particle Green's function,   \textit{susc} to the two-point susceptibilities ,\textit{hedin} to the three-particle susceptibilities, and \textit{vertex} to the four-point susceptibilities.  The specifiers \textit{\_ph} and \textit{\_pp} refer to the particle-hole and particle-particle channels. The asymptotic kernels can only be computed if all two-particle susceptibilities are measured. 

\begin{table} [hb]
\caption{Miscellaneous parameters which are not in a control block. Required.} \label{tab:params:misc}
\footnotesize
 \begin{tabular}{p{4cm} p{11cm}}
\hline  
\textbf{beta}  (real, none)& Inverse temperature of the simulation \\
\textbf{mu}  (real, none)& Chemical potential of the impurity. \\
\textbf{sim per device} (int, 1) & Number of simulations to run on each available GPU. \\
\textbf{thermalisation time} \newline (int, none)& Number of  minutes to run CTQMC (to reach physical configurations) and Wang-Landau (to determine $\eta_{\mathcal{O}}$) before beginning measurement.\\
\textbf{measurement time} \newline (int, none)& Number of minutes to continue CTQMC after thermalisation is complete, during which the Markov chains are sampled and observables are measured. \\
\textbf{thermalisation steps} \newline (int, none)& Number of steps to run CTQMC (to reach physical configurations) and Wang-Landau (to determine $\eta_{\mathcal{O}}$) before beginning measurement. (Overrides thermalisation time.) Note that each simulation (MPI worker and GPU stream) will require (sometimes drastically) different amounts of time to advance a given number of steps, so computational time is wasted when using this option. \\
\textbf{measurement steps} \newline (int, none)& Number of minutes to continue CTQMC after thermalisation is complete, during which the Markov chains are sampled and observables are measured. (Overrides measurement time.) Note that each simulation (MPI worker and GPU stream) will require (sometimes drastically) different amounts of time to advance a given number of steps, so computational time is wasted when using this option.\\
\textbf{seed}  (real, 41085)& Pseudo random number generator (Mersenne Twister 19937) seed\\
\textbf{seed inc}  (real, 857)& Each Markov chain uses the random seed \verb|(seed)|$+n$\verb|(seed inc)|, where $n$ is the index of the simulation.\\
expansion historgram  \newline (boolean, true)& Accumulate a histogram of the expansion order\\
\textbf{trunc dim}  (integer, $\infty$)& Truncates the operator matrices at $i<$\verb|(trunc dim)|. Truncation helps with memory issues and accelerates the simulation, but the simulation is no longer numerically exact. Moreover, the improved estimators may no longer provide the  same answer as the non-improved estimators. Use with care.\\
\hline
\end{tabular}
\end{table}


\begin{table}
\caption{The local Hamiltonian parameter block, ``hloc". Required.}\label{tab:params:hloc}
\footnotesize
 \begin{tabular}{p{4cm} p{11cm}}
\hline  
\textbf{one-body}  \newline (matrix[real], none)& The one-body energy matrix of the impurity, i.e., the $t_{ij}$ from Eq. \ref{equ:ImpurityHamiltonian}. The matrix is written as an array of arrays, each array having $n$ entries, where $n$ is the number of spin-orbital flavors. \\
\textbf{two-body} \newline  (array[real], none)& The static two-body interaction matrix, $V_{ijkl}$, flattened along $i\rightarrow j \rightarrow k \rightarrow l$. \\
\textbf{two-body }  (dictionary)& Instead of entering $V_{ijkl}$ by hand, one can provide a Slater-Condon or Kanamori parameterisation in the \verb|two-body| block. If one uses this block, the local one-particle basis set must also be provided. (See the \verb|basis| block.) \\
~---~ \textbf{parameterisation}  \newline (string)& ``slater-condon'' or ``kanamori" \\
~---~ \textbf{U ,J, Uprime}  \newline (real, none)& The Kanamori parameters (kanamori). By default, $U'=U-2J$. \\
~---~  \textbf{F0, F2, F4, ...  }\newline (real, none)& The $l+1$ 	Slater-Condon parameters (slater-condon) \\
~---~  \textbf{approximation } \newline (string,``none")& ``none" or ``ising'', where ``ising'' keeps only the  $V_{\alpha\beta\beta\alpha}$ and $V_{\alpha\beta\alpha\beta}$ components, and ``none'' keeps all components of $V$. \\
\hline
\end{tabular}
\end{table}

\begin{table}
\caption{The local one-particle basis parameter block, ``basis'', which is required if the two-body interaction matrix is not entered by hand.}\label{tab:params:basis}
\footnotesize
 \begin{tabular}{p{4cm} p{11cm}}
\hline  
\textbf{type}   (string, ``generic'')&  ``generic'', ``product'', or ``coupled''. The underlying basis set. See \ref{app:basis}.\\
\textbf{orbitals}   (real, none)&  The number of orbitals (generic) \\
\textbf{orbitals}  (string, none)& The orbital momentum: $s$ ($l=0$), $p$ ($l=1$), $d$ ($l=2$), or $f$ ($l=3$) (product, coupled) \\
\textbf{transformation}  \newline (matrix[real], $I$)&  Transformation matrix which projects or rotates the basis such that $c^\dagger_i = \sum_j U_{ij} \tilde{c}_j^{\dagger}$. \\
\hline
\end{tabular}
\end{table}

\begin{table}
\caption{The hybridisation parameter block, ``hybridisation'. Required. '}\label{tab:params:hybridisation}
\footnotesize
 \begin{tabular}{p{4cm} p{11cm}}
\hline  
\textbf{functions } (string, none)& The name of the file containing the hybridisation functions, e.g., ``hybridisation.json''. This file contains a json dictionary describing the hybridisation functions $\Delta_{ij}(i\nu)$. \\
\textbf{matrix}  \newline (matrix[string], none)& A matrix of keys which relates the $\Delta_{ij}(i\nu)$  provided in the \verb|hybridisation.json| file to the indices $i$ and $j$ of the associated impurity flavors. If a non-generic basis is used, one must be careful that the hybridisation matrix is ordered according to the enumeration of that basis, as described in \ref{app:basis}. If $\Delta_{ij}(i\nu)=0$, the matrix entry must be the empty string ``''. See Sec. \ref{sec:Examples} for examples.\\
\hline
\end{tabular}
\end{table}



\begin{table}
\caption{The partition space measurement block, ``partition''. Required.}\label{tab:params:partition}
\footnotesize
 \begin{tabular}{p{4cm} p{11cm}}
\hline  
\textbf{green basis}  \newline (string, matsubara)& The basis, ``matsubara'' or ``legendre'', in which the green's function is accumulated.\\
\textbf{green bulla }\newline (boolean, true)& Use the improved estimator for the green's function. \\
\textbf{green matsubara cutoff} \newline (real, none)& The largest frequency to measure for the Green's function, $i\nu_n<2\pi n/\beta$ \\
\textbf{green legendre cutoff} \newline (real, none)& The number of legendre components to accumulate \\
\textbf{occupation susceptibility direct } (boolean, false)& Susceptibilities for the orbital occupations $\chi_{iijj}$ are measured. \\
\textbf{occupation susceptibility bulla}  (boolean, true)& The improved estimators are used to accumulate the $\chi_{iijj}$ \\
\textbf{quantum numbers} \newline (dictionary)& The quantum numbers for which susceptibilities should are measured. Written as either arrays, $q_{n}$, $n=0,1,..,n_{\mathrm{orbitals}}$, or as an empty dictionary, $q={}$, for common quantum numbers for which \ctqmcname{} can auto-generate the correct arrays. Currently implemented are the particle number, $N$, $z$-component of the total  spin, \verb|Sz|, or angular momentum, \verb|Jz|, or the total spin squared, \verb|S2|, or total angular momentum squared, \verb|J2|. Note that the supplied quantum numbers do not have an effect on the CTQMC algorithm or division of the Hilbert space into invariant spaces. Instead, they direct \ctqmcname{} to measure a particular set of susceptibilities (see the option \verb|quantum number susceptibiility|) or associate a set of names with a set of quantum numbers for use during post-processing (see the option \verb|probabilities|). \ctqmcname{} will check that the supplied quantum numbers are actually quantum numbers of the local Hamiltonian. \\
\textbf{quantum number susceptibility}  \newline (boolean, false)& The susceptibility for the quantum numbers, $\chi_{I}$, are accumulated. See Sec. \ref{sec:Examples} for an example.\\
\textbf{susceptibility cutoff}  \newline (real, none)& The largest frequency to measure for the susceptibilities, $i\omega_n<2\pi n/\beta$ \\
\textbf{density matrix precise} \newline (boolean, false)& Measure the impurity reduced density matrix in a more accurate, but more expensive manner. Improves static observable estimators and high-frequency tail fits but costs some computational time during sampling. (Not implemented for GPUs.)\\
\textbf{probabilities} \newline (array[string], empty) & An array listing the names of the quantum number for which the probability of occupancy should be computed during post-processing. The keyword "energy" can also be included, so that the energy of the associated state is output. Used to generate histograms of the valence occupancy. The output is sorted in ascending order across all quantum numbers.  For example, \verb|"probabilities": ["energy","N"]| directs \ctqmcname{} to output the energy, number of electrons, and probability of occupancy of all irreducible states of the local Hamiltonian. The output list will be ordered from lowest-to-highest energy. If two states have the same energy, they will be ordered from lowest-to-highest number of electrons.  \\
\textbf{sweepA } (real, 50)& Number of steps taken by Markov chain in  partition function space before sampling those observables which are computationally inexpensive to sample (Susceptibilities and Green's functions). \\
\textbf{sweepB}  (real, 250)& Number of steps before sampling those observables which are computationally expensive to sample (Improved estimators and precise density matrix).\\
\hline
\end{tabular}
\end{table}


\begin{table}
\caption{
The two-point worm space measurement blocks, ``green'', ``susc\_ph '', and ``susc\_pp ''. Required for worm measurements of these observables. 
}\label{tab:params:green}
\footnotesize
 \begin{tabular}{p{4cm} p{11cm}}
\hline  
\textbf{basis} \newline (string, ``matsubara'')& Basis, ``matsubara'' or ``legendre'', in which to accumulate the observable \\
cutoff  (string, none)& Number of Matsubara or Legendre components to measure, $n<$\verb|(cutoff)|. \\
\textbf{meas} \newline  (array[string], \newline   [``imprsum''])& Manner, ``'', or ``imprsum'', in which to accumulate the observable, i.e., with or without the improved estimator. The improved estimators are not implemented for \verb|susc_ph| or \verb|susc_pp| worm spaces. \\
\textbf{sweep}  (real, 50)& Number of steps between samples of the worm space.\\
\hline
\end{tabular}
\end{table}


\begin{table}
\caption{
The three- and four-point worm space measurement blocks, ``hedin\_ph '', ``hedin\_pp '', and ``vertex''.  Required for worm measurements of these observables. 
}\label{tab:params:vertex}
\footnotesize
 \begin{tabular}{p{4cm} p{11cm}}
\hline  
\textbf{basis}  \newline (string, ``matsubara'')& Basis, ``matsubara'' or ``legendre'', in which to accumulate the observable \\
\textbf{fermion cutoff}  \newline (int, none)& Number of fermionic Matsubara or Legendre components to measure, $|n|<$\verb|(fermion cutoff)| \\
\textbf{boson cutoff}  \newline (int, none)& Number of fermionic Matsubara or Legendre components to measure, $m<$\verb|(boson cutoff)|.  \\
\textbf{matsubara cutoff}  \newline (int, 50)& Number of fermionic Matsubara components to compute during post-processing when measured in the mixed Legendre-Fourier basis \\
\textbf{meas}  \newline (array[string], \newline   [``imprsum''])& Manner, ``'', or ``imprsum'', in which to accumulate the observable, i.e., with or without the improved estimator. \\
\textbf{sweep}  (real, 50)& Number of steps between samples of the worm space. \\
 full  (boolean, false)& Evaluate the corresponding full vertex function during post-processing (only implemented for \verb|vertex|)\\
\hline
 \end{tabular}
 \end{table}


\begin{table}
\caption{The asymptotic kernel parameter block, ``kernels''. Required for computation of kernels.}\label{tab:params:kernels}
\footnotesize
 \begin{tabular}{p{4cm} p{11cm}}
\hline  
 \textbf{full}  (boolean, false)& Compute the full vertex using the asymptotic kernel functions during post-processing. \\
\textbf{fermion cutoff} \newline (int, none)& Number of fermionic Matsubara components for which to compute the asymptotic vertex, $|n|<$\verb|(fermion cutoff)|. \\
 \textbf{boson cutoff}  (int, none)& Number of bosonic Matsubara components for which to compute the asymptotic vertex, $m<$\verb|(bosono cutoff)|. \\
 \textbf{asymptotic cutoff}  \newline (int, 10)& Condition for replacing the measured vertex with asymptotic vertex, \verb|(asymptotic cutoff)|$^4\geq \frac{\beta^4}{\pi^4} \nu(\nu-\omega)\nu'(\nu'-\omega)$\\
\hline
\end{tabular}
 \end{table}

\normalsize

\clearpage
\newpage

==> Src/InstallationAndUsage_copy.tex <==
In this section, we describe how one can acquire, install, and use \ctqmcname. \ctqmcname{} is written in C++11 and CUDA, and uses BLAS and LAPACK libraries. It has been tested with GNU, intel, and clang compilers. 

\subsection{Download}

\ctqmcname{} is an open source code distributed under the GNU General Public Licence 3.0 (GPL). It is a part of the COMSUITE package\\ (\verb|https://www.bnl.gov/comscope/software/comsuite.php|), and can therefore be downloaded from the COMSUITE github page\\ (\verb|https://github.com/comscope/comsuite/tree/master/ComCTQMC|). Alternately, one can contact the authors for the current version of \ctqmcname. 

\subsection{Install}

To build \ctqmcname, one must first decompress the downloaded \ctqmcname{} archive. Typically, \ctqmcname{} will be bundled in an archive like \verb|ComCTQMC.tar.gz|. Therefor, one should navigate to the location where this archive resides and execute
\begin{verbatim}
$ tar xvfz ComCTQMC.tar.gz
\end{verbatim}
where \verb|$| is the command line prompt. Then, one must navigate into the extracted directory.
\begin{verbatim}
$ cd ComCTQMC
\end{verbatim}
In this base directory is the file  \verb|Arch.mk| which specifies the compiler options. While default options are setup here, one should manually specify which compiler and libraries one will use. (See the file \verb|Arch.mk| for further information.) 

Once \verb|Arch.mk| has been setup, one must build the CTQMC and post-processing codes. To do so, navigate to the \verb|CTQMC| directory for either the GPU accelerated version (if the system has CUDA enabled GPUs) or the non-accelerated version
\begin{verbatim}
(GPU Accelerated)	$ cd CTQMC/GPU
(Otherwise)				$ cd CTQMC/CPU
\end{verbatim}
and then build the code
\begin{verbatim}
$ make
\end{verbatim}
The post-processing  code \verb|EvalSim| is similarly built:
\begin{verbatim}
$ cd ../../EvalSim
$ make
\end{verbatim}

\subsection{Execute}

To run \ctqmcname, one must first run CTQMC code \verb|CTQMC| and then run the post-processing code \verb|EvalSim|. To do so from the base directory, one would type 
\begin{verbatim}
(GPU Accelerated)	$ CTQMC/GPU/CTQMC params
								$ EvalSim/EVALSIM params
								
(Otherwise)				$ CTQMC/GPU/CTQMC params
								$ EvalSim/EVALSIM params
\end{verbatim}
where the control file is named \verb|params.json|. 

\subsection{Input and output fiiles}


The input and output files are written in the JSON (JavaScript Object Notation) format\footnote{\url{https://www.json.org/}}. Briefly, this format presents a dictionary pairing keys with data.  An entry can store integer, real number, string, boolean,  array (of those types), or another dictionary entry. The order of the dictionary entries does not matter. We will refer to a the highest level entry in the JSON dictionary as a block. Let us describe the input files required by and then output files produced by \ctqmcname{}. 

The following input files are required by \ctqmcname{}:
\begin{enumerate}
\item \verb|params.json|: The control file describing the simulation, the quantum impurity, the desired measurements and worms, and the system architecture.
\item \verb|hybridisation.json|: The hybridisation functions.
\item \verb|dynamical.json| (optional): The dynamical part of the two-body interaction. This is not required if there is no dynamical part. 
\item \verb|config_n.json| (restart): The state of the Markov chain \verb|n| from which to resume a simulation. This can be used to continue a simulation or to reduce thermalisation times.  (Produced by \ctqmcname.)
\item \verb|params.meas.json| (restart): The state of the estimators at the end of the previous run. Required to automatically continue the simulation and refine the estimators.   (Produced by \ctqmcname.) 
\item \verb|WangLandau.meas.json| (restart): The number of steps taken in each configuration space and the associated renormalization constants, $\eta_{\mathcal{O}}$, at the end of the previous run. Required to continue the simulation or avoid re-computing the renormalization constants.  (Produced by \ctqmcname.)
\end{enumerate}

After completion, \ctqmcname{} produces the following output files:
\begin{enumerate}
\item \verb|config_n.json|:  The state of the Markov chain \verb|n|.
\item  \verb|wanglandau.json|: The number of steps taken in each configuration space and the renormalization constants
\item  \verb|params.meas.json|: Raw measurements needed to compute observables
\end{enumerate}

The post-processing code takes these files and produces the following file:
\begin{itemize}
\item  \verb|params.obs.json|: The observables, e.g., the self-energy, four point vertex, susceptibilities, and green's functions. 
\end{itemize}

\subsubsection{Input Parameters}

Here we describe the many input parameters in the \verb|params.json| file. As noted previously, these parameters are organized in blocks within the parameter file. We will mirror that organization here, first describing the higher level purpose of that block and then subsequently listing and describing the individual fields within the block. The data type will be given in parenthesis after the name of the field. The default value will be given   after the data type. If there  is no default value, we will write \verb|none|. 

Let us begin. We will start with the miscellaneous parameters which do not fit into a block, and then move onto the major blocks. 

\small
\begin{itemize}
\item beta (real, none): Inverse temperature of the simulation
\item mu (real, none): Chemical potential of the impurity. 
\item thermalisation time (int, none): Number of  minutes to run CTQMC (to reach physical configurations) and Wang-Landau (to determine $\eta_{\mathcal{O}}$) before beginning measurement.
\item measurement time (int, none) Number of minutes to continue CTQMC after thermalisation is complete, during which the Markov chains are sampled and observables are measured. 
\item seed(real, 41085) Pseudo random number generator (Mersenne Twister 19937) seed
\item seed inc (real, 857) Each MPI image uses a seed \verb|(seed)|$+r$\verb|(seed inc)|, where $r$ is the rank of the image. 
\item expansion historgram (boolean, true) Accumulate a histogram of the expansion order
\item  truc dim (integer, $\inf$) Truncates the operator matrices at $i<$\verb|(trunc dim)|. Tuncation helps with memory issues and accelerates the simulation, but the simulation is no longer numerically exact. Moreover, the improved estimators may no longer provide the  same answer as the non-improved estimators. Use with care. 
\item hloc: A description of the local, impurity Hamiltonian.
\begin{itemize}
\item one-body (array[array[real]], none): The one-body energy matrix of the impurity, i.e., the $t_{ij}$ from Eq. \ref{equ:LocHam}). The matrix is written as an array of arrays, each array having $n$ entries, where $n$ is the number of spin-orbital flavors. 
\item two-body (array[real], none): The static two-body interaction matrix, $V_{ijkl}$, flattened along $i\rightarrow j \rightarrow k \rightarrow l$.
\item two-body (dictionary): Instead of entering $V_{ijkl}$ by hand, one can provide a Slater-Condon or Kanamori parameterisation block. If one uses this block, the local one-particle basis set must also be provided. (See the \verb|basis| block.) 
\begin{itemize}
\item parameterisation (string): ``slater-condon'' or ``kanamori" (no capitalization). 
\item U ,J, Uprime (real, none, none $U'=U-2J$): The Kanamori parameters (kanamori)
\item F0, F2, F4, ... (real, none): The $l+1$ 	Slater-Condon parameters (slater-condon)
\item approximation (string,``none"): ``none" or ``ising'', where ``ising'' keeps only the  $V_{\alpha\beta\beta\alpha}$ and $V_{\alpha\beta\alpha\beta}$ components, and ``none'' keeps all components of $V$.
\end{itemize}
\end{itemize}
\item basis: A description of the local, one-particle basis. A generic (kanamori), product (slater-condon), and spin-orbit coupled (slater-condon) basis sets are implemented. 
\begin{itemize}
\item type (string, ``generic'': ``generic'', ``product'', or ``coupled''.
\item orbitals (real, none): The number of orbitals (generic).
\item orbitals (string, none): The orbital momentum: $s$ ($l=0$), $p$ ($l=1$), $d$ ($l=2$), or $f$ ($l=3$) (product, coupled)
\item transformation (array[array[real]], identity matrix): Transformation matrix which projects or rotates the basis such that $c^\dagger_i = \sum_j U_{ij} \tilde{c}_j^{dagger}$. 
\end{itemize}
\item hybridisation: A description of the hybridisation between the impurity orbitals and the bath
\begin{itemize}
\item functions (string, none): The name of the file containing the hybridisation functions, e.g., ``hybridisation.json''. This file contains a json dictionary describing the hybridisation functions $\Delta_{ij}(i\nu)$. 
\item matrix (array[array[string]], none): A matrix which relates the $\Delta_{ij}(i\nu)$  provided in the \verb|hybridisation.json| file to the indices $i$ and $j$.  If $\Delta_{ij}(i\nu)=0$, the entry is the empty string ``''. See Sec. \ref{sec:examples} for examples. 
\end{itemize}
\item partition: A description of the observables  measured  while in partition space
\begin{itemize}
\item green basis (string, matsubara): The basis, ``matsubara'' or ``legendre'', in which the green's function is accumulated.
\item green bulla (boolean, true): Use the improved estimator for the green's function.
\item green matsubara cutoff (real, none): The largest frequency to measure for the Green's function, $i\nu_n<2\pi n/\beta$
\item occupation susceptibility direct (boolean, false): Susceptibilities for the orbital occupatioins $\chi_{iijj}$ are measured. 
\item occupation susceptibility bulla (boolean, true): The improved estimators are used to accumulate the $\chi_{iijj}$
\item quantum numbers (dictionary): A description of the quantum numbers, $I$, of the Hamiltonian written as arrays $q_{In}$, $n=0,1,..,n_{\mathrm{orbitals}}$. $I=$\verb|N|, the total charge, is used by default. \verb|Sz|, total spin up or down is also implemented. 
\item quantum number susceptibility (boolean, false): The susceptibility for the quantum numbers, $\chi_{I}$, are accumulated. See Sec. \ref{sec:examples} for an example. 
\item  susceptibility cutoff (real, none): The largest frequency to measure for the susceptibilities, $i\omega_n<2\pi n/\beta$
\item density matrix precise (boolean, false): Measure the impurity reduced density matrix in a more accurate, but more expensive manner. Improves static observable estimators and high-frequency tail fits but costs some computational time during sampling.
\item sweepA (real, 50): Number of steps taken by markov chain in  partition function space before sampling those observables which are computationally inexpensive to sample (Susceptibilities and Green's functions).
\item sweepB (real, 250): Number of steps before sampling those observables which are computationally expensive to sample (Improved estimators and precise density matrix).
\end{itemize}
\item \verb|green, susc_ph, susc_pp|: A description of the worm space and its sampling. Green referes to the one-particle Green's function. \verb|susc| refers to the two-point susceptibilities. \verb|_ph| and \verb|_pp| refer to the particle-hole and particle-particle channels. These observables are only measured if the associated block is included. 
\begin{itemize}
\item basis (string, ``matsubara''): Basis, ``matsubara'' or ``legendre'', in which to accumulate the observable
\item cutoff (string, none): Number of Matsubara or Legendre components to measure, $n<$\verb|(cutoff)|. 
\item meas (array[string], [``imprsum'']): Manner, ``'', or ``imprsum'', in which to accumulate the observable, i.e., with or without the improved estimator. The improved estimators are not implemented for \verb|susc_ph| or \verb|susc_pp| worm spaces. 
\item  sweep (real, 50): Number of steps between samples of the worm space.
\end{itemize}
\item \verb|hedin_ph, hedin_pp, vertex|: A description of the worm space and its sampling. Hedin refers to a three point susceptibility. The \verb|_ph| and \verb|_pp| indicates that these will be measured in the particle-hole and particle-particle channels. Vertex refers to a four-point susceptibility. These observables are only measured if the associated block is included. 
\begin{itemize}
\item basis (string, ``matsubara''): Basis, ``matsubara'' or ``legendre'', in which to accumulate the observable
\item fermion cutoff (int, none): Number of fermionic Matsubara or Legendre components to measure, $|n|<$\verb|(fermion cutoff)|. 
\item boson cutoff (int, none): Number of fermionic Matsubara or Legendre components to measure, $m<$\verb|(boson cutoff)|. 
\item matsubara cutoff (int, 50): Number of fermionic Matsubara components to compute during post-processing when measured in the mixed Legendre-Fourier basis, 
\item meas (array[string], [``imprsum'']): Manner, ``'', or ``imprsum'', in which to accumulate the observable, i.e., with or without the improved estimator. 
\item  sweep (real, 50): Number of steps between samples of the worm space.
\item full (boolean, false): Evaluate the corresponding full vertex function during post-processing (only implemented for Vertex)
\end{itemize}
\item kernels: A description of the kernel functions used to compute the asymptotics of the four-point full vertex. These are computed during post-processing and are not accumulated during the main CTQMC algorithm. All two- and three-point susceptibilities must be measured for \ctqmcname{} to compute the asymptotic kernels. The bosonic and fermionic cutoff frequencies for every two and three-point susceptibility must be the same. The Hedin susceptibilities must be measured using the improved estimators. The kernels are only computed if this block is present in the 
\begin{itemize}
\item full (boolean, false): Compute the full vertex using the asymptotic kernel functions during post-processing. 
\item fermion cutoff (int, none): Number of fermionic Matsubara components for which to compute the asymptotic vertex, $|n|<$\verb|(fermion cutoff)|. 
\item boson cutoff (int, none): Number of bosonic Matsubara components for which to compute the asymptotic vertex, $m<$\verb|(bosono cutoff)|. 
\item asymptotic cutoff (int, 10): Condition for replacing the measured vertex with asymptotic vertex, \verb|(asymptotic cutoff)|$^4\geq \frac{\beta^4}{\pi^4} \nu(\nu-\omega)\nu'(\nu'-\omega)$
\end{itemize}
\end{itemize}

\normalsize






==> Src/Structure.tex <==
In this section, we briefly outline the structure of \ctqmcname. It is composed of two main components, the main Quantum Monte Carlo code, \verb|CTQMC|, and the post-processing code, \verb|EvalSim|. The CTQMC code proceeds through four phases: Initialization, thermaliziation, measurement, and finalization, as shown in Fig. \ref{fig:structure}. Let us briefly discuss each of these in turn. 

\begin{figure}
\centering
\includegraphics[scale=1]{fig/CodeStructure.eps}
\caption{Simplified structure of \ctqmcname. During initialization, the major objects of the code are constructed. We divide these into the objects which keep track of the configuration, the observables, and the normalization between worm spaces. During thermalization, we equilibrate the configuration and compute the volume re-normalization factors, $\eta_{\mathcal{O}}$. The final result is broadcast to all MPI images. (Communication events are italicized.)
During measurement, the configuration spaces are sampled by the various observable objects as the Markov chain is updated, while $\mathcal{W}$ keeps track of the number of steps taken in each space. During finalization, some post-processing might be done on each observable before the results are averaged across the MPI images and then written to file. 
}
\label{fig:structure}
\end{figure}

\subsubsection{Initialization}
The major tasks of the initialization phase are to read in and interpret the control file, construct the objects which will be used throughout the CTQMC simulation, and initiate the parallel computing and GPU acceleration frameworks as discussed in more detail in Sec. \ref{sec:Implementation}. In particular, a number of Markov chains will be generated. Each Markov chain keeps track of the configuration, the observables, and the renormalization information. 

In \ctqmcname, the configuration information is divided into general information and information related to the bath, the static impurity interactions, and dynamical impurity interactions. \ctqmcname{} also creates a list of updates which will be used to advance the Markov chain.  

Similarly, a list of observables are constructed for both partition space and worm space measurements. The worm space measurements are generalized according to the number of fermionic and bosonic times ($\tau_i^{(f)}$ and $\tau_j^{(b)}$) associated with the observable as well as the basis functions the user requests for their accumulation. In contrast, the partition space measurements are specialized according to their unique requirements.

Finally, the renormalization object, $\mathcal{W}$, is used to keep track of and update the volume renormalization constants associated with each worm space, $\eta_{mathcal{O}}$, and the number of steps taken in each configuration space $N_{\mathcal{O}}$. 

\subsubsection{Thermalization}
During the thermalization phase, \ctqmcname, the Markov Chains are advanced by selecting a random update from the list of update objects. The proposed Metropolis-Hasting acceptance ratio (\ref{sec:metropolis-hasting} is then evaluated in parts by each configuration object, which use those optimizations discussed in Sec. \ref{sec:Implementation}. 

Every step, the Wang Landau algorithm is used to renormalize the volume of the various configuration spaces. This continues until the simulation time, $t$, reaches the thermalization time, $t_{\mathrm{thermalization}}$, specified by the user.  This time should be sufficient for $\eta_{\mathcal{O}}$ to converge and for the Markov chains to thermalize, i.e., equilibrate.\footnote{The results should not depend on the thermalizatioin time. If one finds that they do, nicrease the thermalization time.}

At the end of the thermalization phase, the $\eta_{\mathcal{O}}$ is averaged across all MPI images. The result is broadcast back to every image for use in the subsequent measurement phase. If no thermalization phase occurs, $\eta_{\mathcal{O}}$ is taken from a restart file or, if that does not exist, the user input. If \ctqmcname{} cannot find any $\eta_{mathcal{O}}$ and the thermalization phase does not occur, all $\eta_{mathcal{O}}$ are set to unity. 

\subsubsection{Measurement}
During the measurement phase, \ctqmcname{} not only advances the Markov chain, as in the thermalization phase, but it also samples the Markov chain periodically. Ideally, these samples are not autocorrelated. (Tools are provided to sample autocorrelation, but \ctqmcname{} does not yet automatically determine the ideal sampling period. Instead the user must supply this period via the \verb|sweep| keyword.) 
After a large number of samples have been taken, they are stored in a more processed form.  The number of steps taken in each configuration space is also recorded. Every measurement taken during this phase is associated with the markov chain from which it is taken. That is, there is no communication between Markov chains.

\subsection{Finilazation}
During finalization, the measurements taken from every Markov chain is collected. Those quantities which are a Monte-Carlo average are averaged across every Markov chain with a weight equal to the number  of samples taken by that Markov chain.  Then, the measurements and information required for a restart are written to file. Similarly, the number of steps taken in each configuration space are summed across Markov chains and written to file, along with the associated volume renormalization constant. 







